Efficient Multiple Temporal Network Kernel Density Estimation

Kernel density estimation (KDE) has become a popular method for visual analysis in various fields, such as financial risk forecasting, crime clustering, and traffic monitoring. KDE can identify high-density areas from discrete datasets. However, most existing works only consider planar distance and spatial data. In this paper, we introduce a new model, called TN-KDE, that applies KDE-based techniques to road networks with temporal data. Specifically, we introduce a novel solution, Range Forest Solution (RFS), which can efficiently compute KDE values on spatiotemporal road networks. To support the insertion operation, we present a dynamic version, called Dynamic Range Forest Solution (DRFS). We also propose an optimization called Lixel Sharing (LS) to share similar KDE values between two adjacent lixels. Furthermore, our solutions support many non-polynomial kernel functions and still report exact values. Experimental results show that our solutions achieve up to 6 times faster than the state-of-the-art method.

==> head.tex <==
\usepackage{booktabs} % format tables
\usepackage{times} % times font can reduce page length
\usepackage{color} % color figures
\usepackage{balance} %balance the end of the draft
\usepackage{url} 
\usepackage{tabularx}
\usepackage{siunitx} %unit package for special unit symbols
\usepackage{epstopdf} % convert eps figures to pdf
\usepackage{epsfig,tabularx,subfigure,multirow, graphicx}
\usepackage{enumitem}
\usepackage{caption}
\captionsetup[figure]{font=small,skip=0ex, belowskip=-5pt}
\captionsetup[table]{font=small,skip=-2pt}


%\usepackage[sorting=none]{biblatex}
\setlength{\textfloatsep}{2ex}% Remove vertical space below Algrithm block
%\usepackage[bookmarks=false]{hyperref} % add hyper reference to citations and references

\usepackage{amsthm,amsmath, amssymb}  % support for mathematic symbols

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\SetKwRepeat{Do}{do}{while}% add do-while sentences
\newcommand\mycommfont[1]{\scriptsize\ttfamily{#1}} %adjust the font size of comments
\SetCommentSty{mycommfont}


\newcommand{\stitle}[1]{\vspace{1ex} \noindent{\bf #1}}
\long\def\comment#1{}

\setlength{\algomargin}{1em} %adjust the side margin of algorithm blocks
%\setlength{\textfloatsep}{1ex} %adjust the space above and below the float block, including algorithms, figures, tables

\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\nop}[1]{}

\newcommand{\figureTopMargin}{\vspace{-3ex}}
\newcommand{\figureCaptionMargin}{\vspace{-1ex}}
\newcommand{\figureBelowMargin}{\vspace{-2ex}}
\newcommand{\tableTopMargin}{\vspace{-4ex}}
\newcommand{\tableBelowMargin}{\vspace{-3ex}}
\newcommand{\algoTopMargin}{\vspace{-3ex}}
\newcommand{\algoBelowMargin}{\vspace{-3ex}}
\newcommand{\itemMargin}{\vspace{-1ex}}

\newcommand\abs[1]{\left\lvert #1 \right\rvert}


%%%%%%%uncomment below commands to enable related blocks
\newtheorem{theorem}{\bf Theorem}[section]
\newtheorem{lemma}{\bf Lemma}[section]
\newtheorem{corollary}{\bf Corollary}[section]
\newtheorem{example}{\bf Example}

\theoremstyle{remark}
\newtheorem{remark}{\bf Remark}[section]

\theoremstyle{definition}
\newtheorem{definition}{\bf Definition}


